Autoregressive 3D Shape Generation via Canonical Mapping

With the capacity of modeling long-range dependencies in sequential data, transformers have shown remarkable performances in a variety of generative tasks such as image, audio, and text generation. Yet, taming them in generating less structured and voluminous data formats such as high-resolution point clouds have seldom been explored due to ambiguous sequentialization processes and infeasible computation burden. In this paper, we aim to further exploit the power of transformers and employ them for the task of 3D point cloud generation. The key idea is to decompose point clouds of one category into semantically aligned sequences of shape compositions, via a learned canonical space. These shape compositions can then be quantized and used to learn a context-rich composition codebook for point cloud generation. Experimental results on point cloud reconstruction and unconditional generation show that our model performs favorably against state-of-the-art approaches. Furthermore, our model can be easily extended to multi-modal shape completion as an application for conditional shape generation.

==> 03-Methodology.tex <==
\section{Method}
\input{figures/overview/overview}

Our CanonicalVAE consists of three stages:

\paragraph{\textbf{Stage 1: Point Cloud Canonicalization.}} 
Our point cloud canonicalization stage aims to canonicalize a point cloud by structuralizing and factorizing a point cloud. To that end, we learn two functions: an canonical mapping function and a canonical grouping function. The canonical mapping function conditions on an input point cloud $x$ and builds dense correspondence between $x$ and a canonical sphere. The canonical sphere then served as a medium to implicitly structuralize each input point clouds. To further factorize the structure, we learn a canonical grouping function to segment the canonical sphere into groups.

\paragraph{\textbf{Stage 2: Point Cloud Quantization.}}
We train a vector-quantized variational autoencoder to compress each canonicalized point cloud into discretized group tokens.  

\paragraph{\textbf{Stage 3: Vector-quantized Point Cloud Modeling.}}
We train a Transformer model to predict the discretized group tokens autoregressively. For unconditional shape synthesis, we train a decoder-only Transformer model to predict the next token. For conditional shape synthesis, we extract features from the conditional input and use the features as the embeddings of conditional tokens in the Transformer model.
\\
We illustrate the overview of the proposed \modelName in Figure~\ref{fig:overview}. The following subsections describe each stage in further detail.



\subsection{Point Cloud Canonicalization}\label{sec:pcl-canonicalization}

\subsubsection{Canonical Mapping function}\label{sec:pcl-canonicalization-cmf}
Recent work~\cite{cheng2021learning,deprelle2019learning} show that dense correspondence between shapes can be implicitly build by learning to deform point clouds from a shared primitive structure(e.g., 2D grid, 3D sphere). 
Motivated by these approaches, we train a canonical autoencoder to learn the mapping function between a canonical sphere and point clouds. Our encoder follows the architectures as in ~\cite{wang2019dynamic}. Specifically, each point from an input point cloud $x\in\mathcal{R}^{M\times3}$ is represented as a 256-dimensional point-wise feature using 3 layers of EdgeConvs. We then aggregate all point features with max-pooling and a linear layer to generate a 256-dimensional global latent code. Before feeding the global latent into the decoder, we replicate the latent code $M$ times and concatenate the replicated latent matrix $(M, 256)$ with an $(M, 2)$ matrix $\pi$, which contains $M$ uniformly sampled points from a unit sphere. Our decoder follows the two branch structure as in ~\cite{li2021sp}. With the concatenated matrix as input, the decoder first feeds sphere points to a graph attention module to extract point-wise spatial features. On the other branch, we use a nonlinear feature embedding to extract style features from the latent. Then, we use adaptive instance normalization to fuse the local styles with the spatial features. We repeat the process with another round of style embedding and fusion, and then predict a reconstructed point cloud $\hat{x}$ from the fused feature. Finally, a reconstruction loss combining Chamfer Distance and Earth Mover Distance is used to measure the difference between the input point cloud $x$ and the outputted point cloud $\hat{x}$.

\begin{equation}
\mathcal{L}_{CanonicalMapping}= L_{CD}(P, \hat{S}) + L_{EMD}(P, \hat{S})
\label{eq:stage1-1-loss}
\end{equation}

With a pretrained canonical autoencoder, given a point cloud $x$, a canonical sphere $\pi$, we can first obtain $\hat{x}$ which is in $\pi$'s order. Then for arbitrary $q_{i} \in \pi$ we can find its canonical mapping point on $x$ by $\mathop{\arg\min}_{{x}_{j}\in x}  \left\Vert x_{i} - \bar{x}_{j} \right\Vert_2$. Subsequently, we can sort point cloud $x$ following canonical sphere $\pi$'s order by sequentially finding every canonical mapping point in $\pi$. Similarly, we can sort a canonical sphere $\pi$ following a point cloud $x$'s order with each of its inverse canonical mapping point.


\subsubsection{Canonical Grouping Function}\label{sec:pcl-canonicalization-cgf}
A simple way to factorize the canonical sphere into $g$ sub-spaces is to uniformly divide the sphere by sampling $g$ random points on the sphere as center points and perform nearest neighbor search for each point on the canonical sphere. However, this approach do not provide any semantic consistency across all the shape instances. Inspired by recent work on shape structure analysis~\cite{chen2020unsupervised}, we introduce an self-supervised method to learn semantic consistent group representation on the canonical sphere.

With a pretrained canonical mapping function, we can sort a canonical sphere $\pi$ in a point cloud $x$'s order, which we denoted as $\pi_{\pi\rightarrow x}$. Then we apply a shared multi-layer perceptron (MLP) block followed by a softmax activation function to predict the probability maps $P=\{p_1, p_2, ..., p_m\}$ for each $q_i \in \pi_{\pi\rightarrow x}$. 
The element $p_i^j$ in the probability map $p_i$ indicates the probability of the point $q_i$ being the structure point for the $j^{th}$ group on the canonical sphere. As $\pi_{\pi\rightarrow x}$ and $x$ now shares the same semantic order, we can compute the structure points $K$ predicted for each input shape $x$, where:

\begin{equation}\label{eq:integration}
k_j = \sum_{i=1}^{m} x_i p_i^j  \quad \textrm{with} \quad \sum_{i=1}^{m} p_i^j=1 \quad \textrm{for}  \quad j=1,2,3...g
\end{equation}

In order to learn semantically consistent grouping across the shapes, we optimize a reconstruction loss based on Chamfer distance to constrain the predicted structure points $K$ to be close to each input point cloud $x$.

\begin{equation}
\mathcal{L}_{CanonicalGrouping} =  \mathcal{L}_{CD}(K, x)
\end{equation}

% \begin{equation}\label{eq:general_cd}
% \mathcal{L}_{CanonicalGrouping} =  \sum_{k_g \in K} \min_{s_i \in S} \|k_g-s_i\|_2^2 + \sum_{s_i \in S} \min_{k_g \in K} \|k_g-s_i\|_2^2
% \end{equation}

After training, we can then assign the $i^{th}$ point in both $\pi_{\pi\rightarrow x}$ and $x$ with a group index $j$ by $\mathop{\arg\max}_{j} p_i^j$. 


\subsection{Shape Vector Quantization}\label{sec:pcl-quantization}
Our shape quantization stage contains three components, an encoder $E$, a decoder $D$, and a vector quantizer $Q$. Through training a vector quantized autoencoder, we can approximate a point cloud $x$ by $\hat{x} = D(z_{q}, \pi)$ , where $z_{q} \in \mathcal{R}^{g\times 256}$ is the quantized code representing $x$. 

% we first extract 256-dimensional point-wise features from a canonicalized point cloud $x$

To train the vector quantized autoencoder, we first canonicalize the input point cloud $x$ and the sphere points $\pi$ to obtain each of their group index. Then we use an encoder $E$ to extract 256-dimensional point-wise features from cloud $x$.
For point-wise features that shares the same group indices, we apply max-pooling to aggregate them into group features $\hat{z} \in \mathcal{R}^{g \times 256}$.  

We them perform quantization on each group features in $\hat{z}$ onto its closest entry in a codebook $Z$ to get quantized group codes $z_{q}$. Vector quantization suffers from low codebook usage due to the poor initialization of the codebook. If a significant portion of codes are unused, it results in worse reconstructions. Therefore, to encourage codebook utilization, we propose to use stand-alone codebooks for each group. Specifically, $z_{q}$ is calculated by element-wise quantization $Q(\cdot)$ of each group code $\hat{z}^{j}$ onto its closest codebook entry in $z^{j}\subset Z$. Recent work on image vector quantization shows that by keeping the dimension of lookup space in a lower dimension can improve reconstruction quality. Thus, we employ dimension reduction on the encoded $\hat{z}^{j}$, so that the lookup space is in a lower dimension. After the encoded $\hat{z}^{j}$ is matched with a lower-dimensional code in the codebook, we project the code back to the high-dimensional embedding space to get $z_{q}^{j}$.

Finally, to decode $\hat{x}$ from $z_{q}$, we concatenate each point in $\pi$ with a quantized group code based on its group index and feed the concatenated matrix to the decoder. Note that for both $E$ and $D$, we use the same network architecture as in Section~\ref{sec:pcl-canonicalization-cmf}. 

The training objective of our shape quantization is defined as follows

\begin{equation}
\begin{aligned}
\mathcal{L}_{Quantization}=\mathcal{L}_{CD}(x,\hat{x}) + \mathcal{L}_{EMD}(x,\hat{x}) & + \left \| sg[E(x)]-z_{q} \right \|_{2}^{2} \\ & + \beta \left \| sg[z_{q}]-E(x) \right \|_{2}^{2}
\end{aligned}
\end{equation}

$\mathcal{L}_{CD}$ and $\mathcal{L}_{EMD}$ are reconstruction loss between input point cloud $x$ and the decoded point cloud $\hat{x}$. $sg[\cdot]$ denotes the stop-gradient operation, $\beta$ is a commonly used hyper-parameter for commitment loss which we set to 1 throughout our experiment.

\subsection{Vector-quantized Shape Modeling}
\label{sec:transformer}
With $E$, $D$, and $Q$ available, we can now represent shapes in terms of a codebook-indices of their encodings. The quantized encoding of a point cloud $x$ is given by $z_{q} = Q(E(x)) \in \mathcal{R}^{g \times 256}$. More precisely, $z_{q}$ is represented as an unordered dictionary of codebook-indices, where the keys are $\forall j \in \{1,…,g\}$ and the value for each group key $j$ is obtained by its index in its corresponding codebook $Z^{j}$. To formulate shape generation as an autoregressive prediction task, we need to flatten the values into a sequence. Since these each of the key corresponds to a distinct area on the canonical sphere, we can sort these keys with its spatial location naturally. Specifically, we traverse the canonical sphere from the pole with a Fibonacci spiral and serialize the group keys. For a point cloud $x$, we obtain a sequence of $s$ with length $G$.

Given indices $s_{<i}$, we train a Transformer model to predict the distribution of possible next indices $s_{i}$. A full representation of a complete shape $s$ can be model as
\begin{equation}
\prod _{i=1}^{G}p(s_{i} | s_{1},s_{2},...,s_{i-1})
\end{equation}

The training objective is to minimize the negative log-likelihood by
\begin{equation}
\mathcal{L}_{Transformer}=\mathbb{E}_{x\mathtt{\sim}p(x))}\left [ -\log p(s) \right ]
\end{equation}

The architecture of our Transformer model is similar to the one in [], where the indices are projected into the embedding space at each position together with an additive positional embedding. However, since each of our token indices owns to its own group codebook respectively, we do not use a shared embedding space for all token indices. Instead, each discrete token index has its corresponding embedding space.

\subsubsection{Unconditional Generation}
With a pretrained generative Transformer model, unconditional shape generation is achieved by sampling token-by-token from the output softmax distribution. The sampled tokens are then fed into the decoder to decode output shapes.

\subsubsection{Conditional Generation}
To show the capability of our model for shape synthesis, we further extend the unconditional shape generation with conditional inputs. Specifically, given a condition $c$, we hope to generate a shape satisfying the semantic meaning of $c$. To that end, we first encode the condition $c$ into a feature vector in the same dimension of token embedding, then prepend the feature vector before the first token embedding.

==> figures/completion/completion_long.tex <==
% <left> <lower> <right> <upper>}
\begin{figure}[t]
    \begin{center}
    \newcommand{\sizea}{0.124\linewidth}
    \newcommand{\sizeb}{0.124\linewidth}
    \newcommand{\sizec}{0.124\linewidth}
    \newcommand{\tare}{5cm}
    \newcommand{\tale}{3.5cm}
    \newcommand{\tal}{3.5cm}
    \newcommand{\tab}{2.5cm}
    \newcommand{\tar}{3.5cm}
    \newcommand{\tat}{3cm}
    \newcommand{\tcl}{3.0cm}
    \newcommand{\tcb}{3cm}
    \newcommand{\tcr}{4cm}
    \newcommand{\tct}{4.2cm}
    \newcommand{\thl}{3.0cm}
    \newcommand{\thb}{0.0cm}
    \newcommand{\thr}{3cm}
    \newcommand{\tht}{2cm}
    \setlength{\tabcolsep}{0pt}
    \renewcommand{\arraystretch}{0}
    \begin{tabular}{@{}cccc:cccc@{}}
    
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_8_depth.png}&
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_8_msc_0.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_8_pvd_0.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_8_ours_0.jpg} &
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_depth.png} &
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_msc_0.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_pvd_0.jpg} &
        \includegraphics[width=\sizea, trim={5cm} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_ours_0.jpg} 
        \\
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_8_part.jpg} &
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_8_msc_1.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_8_pvd_1.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_8_ours_1.jpg} &
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_part.jpg} &
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_msc_2.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_pvd_1.jpg} &
        \includegraphics[width=\sizea, trim={5cm} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_ours_2.jpg}
        \\
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_gdt.jpg} &
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_8_msc_2.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_8_pvd_4.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/2_8_ours_3.jpg} &
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_gdt.jpg} &
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_msc_4.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_pvd_3.jpg} &
        \includegraphics[width=\sizea, trim={5cm} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_ours_3.jpg}
        \\
    
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_3_depth.png}&
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_3_msc_0.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_3_pvd_0.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_3_ours_2.jpg} &
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_8_depth.png} &
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_8_msc_1.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_8_pvd_0.jpg} &
        \includegraphics[width=\sizea, trim={5cm} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_8_ours_0.jpg} 
        \\
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_3_part.jpg} &
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_3_msc_3.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_3_pvd_2.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_3_ours_1.jpg} &
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_8_part.jpg} &
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_8_msc_3.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_8_pvd_1.jpg} &
        \includegraphics[width=\sizea, trim={5cm} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_8_ours_1.jpg}
        \\
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_gdt.jpg} &
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_3_msc_2.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_3_pvd_4.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/8_3_ours_3.jpg} &
        \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_gdt.jpg} &
        \includegraphics[width=\sizec, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_8_msc_4.jpg} &
        \includegraphics[width=\sizeb, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_8_pvd_2.jpg} &
        \includegraphics[width=\sizea, trim={5cm} {\tab} {2cm} {\tat},clip]{figures/completion/chair/10_8_ours_3.jpg}
        \\
        Input/GT & MSC & PVD & Ours & Input/GT & MSC & PVD & Ours
    \end{tabular}

    \end{center}
    \caption{Multi-modal shape completion results. We shown 4 samples comparing to MSC and PVD. The input depth-map, partial point cloud, and reference ground-truth shape for each sample is shown in the first column, respectively (from top to bottom). 
    }
    \label{fig:completion}
\end{figure}



% % <left> <lower> <right> <upper>}
% \begin{figure}[t]
%     \begin{center}
%     \newcommand{\sizea}{0.124\linewidth}
%     \newcommand{\sizeb}{0.10\linewidth}
%     \newcommand{\sizec}{0.08\linewidth}
%     \newcommand{\tare}{5cm}
%     \newcommand{\tale}{4cm}
%     \newcommand{\tal}{3.5cm}
%     \newcommand{\tab}{3cm}
%     \newcommand{\tar}{3.5cm}
%     \newcommand{\tat}{3.5cm}
%     \newcommand{\tcl}{3.0cm}
%     \newcommand{\tcb}{3cm}
%     \newcommand{\tcr}{4cm}
%     \newcommand{\tct}{4.2cm}
%     \newcommand{\thl}{3.0cm}
%     \newcommand{\thb}{0.0cm}
%     \newcommand{\thr}{3cm}
%     \newcommand{\tht}{2cm}
%     \setlength{\tabcolsep}{0pt}
%     \renewcommand{\arraystretch}{0}
%     \begin{tabular}{@{}cccc:cccc@{}}
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_depth.png}&
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_msc_0.jpg} &
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_pvd_0.jpg} &
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_ours_2.jpg} &
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} 
%         \\
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_part.jpg} &
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_msc_2.jpg} &
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_pvd_1.jpg} &
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_ours_0.jpg} &
%         \\
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_gdt.jpg} &
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_msc_4.jpg} &
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_pvd_3.jpg} &
%         \includegraphics[width=\sizea, trim={\tale} {\tab} {2cm} {\tat},clip]{figures/completion/chair/1_1_ours_3.jpg} &
%         \\
%         Input/GDT & MSC & PVD & Ours & Input/GDT & MSC & PVD & Ours
%     \end{tabular}

%     \end{center}
%     \caption{Generation results. We shown results from PF (PointFlow), SetVAE, DPM, and PVD.
%     }
%     \label{fig:gen}
% \end{figure}


==> figures/overview/overview.tex <==
\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/overview/s1s2_overview.png}
\caption{OV.}
\label{fig:overview}
\end{figure}
